Learning Deep Energy Models: Contrastive Divergence vs. Amortized MLE

We propose a number of new algorithms for learning deep energy models and demonstrate their properties. We show that our SteinCD performs well in term of test likelihood, while SteinGAN performs well in terms of generating realistic looking images. Our results suggest promising directions for learning better models by combining GAN-style methods with traditional energy-based learning.

==> tex/related.tex <==
\section{Related Work}
\label{sec:related}

Generative adversarial network (GAN) and its variants have recently gained remarkable success on generating realistic-looking images 
\citep{goodfellow2014generative, salimans2016improved, radford2015unsupervised, li2015generative,dziugaite2015training,nowozin2016f}.  
All these methods are set up to train latent variable models (the generator) under the assistant of the discriminator.  
Our SteinGAN instead performs traditional MLE training for a deep energy model, 
 with the help of a neural sampler that learns to draw samples from the energy model to approximate the likelihood function; 
this admits an adversarial interpretation: we can view the neural sampler as a generator that attends to fool the deep energy model, which in turn serves as a discriminator 
that distinguishes the real samples and the simulated samples given by the neural sampler. 
This idea of training energy models with neural samplers was first discussed by \citet{kim2016deep}; 
one of the key differences is that the neural sampler in \citet{kim2016deep}\todo{and the other energy based method in ICLR?} 
is trained with the help of a heuristic diversity regularizer based on batch normalization, while 
SVGD enforces the diversity in a more principled way. 
%which, without a principled approach for solving Problem~\ref{pro:prob1},  in which the diversity of simulated samples are enforced with a heuristic motivated by batch normalization.  
Another method by \citet{zhao2016energy} also trains an energy score to distinguish real and simulated samples, but within a non-probabilistic framework (see Section~\ref{sec:gan} for more discussion). 
Other more traditional approaches for training energy-based models  \citep[e.g.,][]{ngiam2011learning, xie2016theory} are often based on variants of MCMC-MLE or contrastive divergence \citep{geyer1991markov, hinton2002training, tieleman2008training}, and have difficulty generating realistic-looking images from scratch. 



==> tex/tmp <==
Working on introduction.tex...
1.) Line 2, column 17, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
 \begin{abstract}  We propose a number of new algorithms for lea...
                 ^^                                             

2.) Line 3, column 137, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...y a recent Stein variational gradient descent  (SVGD) algorithm,  including a Stein contrast...
                                                ^^                                             

3.) Line 3, column 156, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...riational gradient descent  (SVGD) algorithm,  including a Stein contrastive divergence (Ste...
                                                ^^                                             

4.) Line 4, column 120, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... SVGD based on their theoretical connections,  and a SteinGAN that  trains an auxiliary gene...
                                                ^^                                             

5.) Line 5, column 20, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...theoretical connections,  and a SteinGAN that  trains an auxiliary generator  to generate th...
                                                ^^                                             

6.) Line 6, column 30, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... SteinGAN that  trains an auxiliary generator  to generate the negative samples in maximum l...
                                                ^^                                             

7.) Line 9, column 4, Rule ID: NON3PRS_VERB[2]
Message: The pronoun 'We' must be used with a non-third-person form of a verb: 'demonstrate'
Suggestion: demonstrate
...t approximates MLE using amortized SVGD.  We demonstrates that our SteinCD trains models with good gen...
                                                ^^^^^^^^^^^^                                             

8.) Line 9, column 99, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ood generalization (high testing likelihood),  while SteinGAN can generate realistic looking...
                                                ^^                                             

9.) Line 12, column 61, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...he performance of our approaches we show that  %a Stein score matching algorithm and a  %We ...
                                                ^^                                             

10.) Line 13, column 40, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...that  %a Stein score matching algorithm and a  %We use an amortized MLE algorithm for traini...
                                                ^^                                             

11.) Line 19, column 15, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... the state-of-the-art results. \end{abstract}   \section{Introduction} %  Energy-based models...
                                                ^^^                                             

12.) Line 22, column 2, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ts. \end{abstract}   \section{Introduction} %  Energy-based models (EBMs) capture dependenci...
                                                ^^                                             

13.) Line 29, column 454, Rule ID: COMMA_PARENTHESIS_WHITESPACE
Message: Put a space after the comma
Suggestion: , ]
...tive surrogate loss functions \citep[see e.g.,][for reviews]{koller2009probabilistic, goodfe...
                                                ^^                                             

14.) Line 30, column 96, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ing} is one of the most important algorithms,   which avoids estimating the normalization con...
                                                ^^^                                             

15.) Line 31, column 67, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ng the normalization constant by optimizing a  contrastive objective that measures how much ...
                                                ^^                                             

16.) Line 32, column 78, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...res how much KL divergence can be improved by  running a small numbers of Markov chain steps...
                                                ^^                                             

17.) Line 36, column 89, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...neralize well (with high testing likelihood),  CD and other traditional energy-based learnin...
                                                ^^                                             

18.) Line 38, column 79, Rule ID: ENGLISH_WORD_REPEAT_RULE
Message: Possible typo: you repeated a word
Suggestion: the
...stances live a relatively low manifold which the the energy-based models can not capture.  %On th...
                                                ^^^^^^^                                             

19.) Line 38, column 79, Rule ID: DT_DT[1]
Message: Maybe you need to remove one determiner so that only 'the' or 'the' is left.
Suggestion: the; the
...stances live a relatively low manifold which the the energy-based models can not capture.  %On th...
                                                ^^^^^^^                                             

20.) Line 40, column 106, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ersarial networks (GAN) \citep{ganpaper XXX},  which, instead of training energy models,  di...
                                                ^^                                             

21.) Line 41, column 42, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...},  which, instead of training energy models,  directly training generate networks that outp...
                                                ^^                                             

22.) Line 42, column 63, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... generate networks that output random samples  to match the observed data %by minimizing a d...
                                                ^^                                             

23.) Line 44, column 45, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... %by minimizing a divergence measure that can  by framing the divergence minimization proble...
                                                ^^                                             

24.) Line 46, column 87, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...volutional networks \citep{cite DCGAN paper},  the prior knowledge of the real-world manifol...
                                                ^^                                             

25.) Line 48, column 12, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...n be incorporated into learning.  %The design  %The problem with GAN, however, is that it ca...
                                                ^^                                             

26.) Line 50, column 77, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...y assign an energy score for each data point,  and can over-fit on a subset of the training ...
                                                ^^                                             

27.) Line 53, column 96, Rule ID: THE_SENT_END[1]
Message: Did you forget something after 'the'?
...nergy-based learning can potentially improve the.  %This makes GAN have relatively low testing...
                                                ^^^^                                             

28.) Line 57, column 56, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...tworks that output samples given random noise  %Although CD can be used for learning  %which...
                                                ^^                                             

29.) Line 58, column 38, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... noise  %Although CD can be used for learning  %which replaces the likelihood obj %Rather th...
                                                ^^                                             

30.) Line 60, column 270, Rule ID: SENTENCE_WHITESPACE
Message: Add a space between sentences
Suggestion:  This
...esponding gradient of the normalization term.This approach is known as contrastive divergence ...
                                                ^^^^                                             

31.) Line 64, column 118, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...r approximate inference \citep{liu2016stein},   we propose a number of new algorithms for tra...
                                                ^^^                                             

32.) Line 65, column 71, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...w algorithms for training deep energy models,  including a \emph{Stein contrastive divergenc...
                                                ^^                                             

33.) Line 66, column 125, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... SVGD based on their theoretical connections,   and a SteinGAN algorithm  that approximates M...
                                                ^^^                                             

34.) Line 67, column 25, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...tical connections,   and a SteinGAN algorithm  that approximates MLE using a sampler (genera...
                                                ^^                                             

35.) Line 69, column 63, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...nCD and SteinGAN exhibit opposite properties,  SteinCD tends to learn models with high testi...
                                                ^^                                             

36.) Line 70, column 101, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ood but can not generate high quality images,  while SteinGAN generates realistic looking im...
                                                ^^                                             

37.) Line 73, column 140, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...h GAN-type methods using energy-based models,  opening the possibility of combining the trad...
                                                ^^                                             

38.) Line 76, column 178, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... approaches for image generative. %\red{todo}  %Instead, we want to demonstrate the possibil...
                                                ^^                                             

39.) Line 77, column 70, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...onstrate the possibility for image generation  %using energy models with traditional MLE app...
                                                ^^                                             

40.) Line 80, column 30, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...le directions.  %The goal of this work is not  %We also propose a  %algorithm that combines ...
                                                ^^                                             

41.) Line 81, column 18, Rule ID: EN_A_VS_AN
Message: Use 'an' instead of 'a' if the following word starts with a vowel sound, e.g. 'an article', 'an hour'
Suggestion: an
...e goal of this work is not  %We also propose a  %algorithm that combines CD and SVGD, which...
                                                ^                                             

42.) Line 81, column 19, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
... goal of this work is not  %We also propose a  %algorithm that combines CD and SVGD, which w...
                                                ^^                                             

43.) Line 85, column 26, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...wang2016steingan}). %The first method is xxx,  %\emph{SteinCD}   %\red{some discussion} %Cri...
                                                ^^                                             

44.) Line 86, column 16, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...). %The first method is xxx,  %\emph{SteinCD}   %\red{some discussion} %Critically, the SVGD ...
                                                ^^^                                             

45.) Line 92, column 6, Rule ID: COMMA_PARENTHESIS_WHITESPACE
Message: Don't put a space after the opening parenthesis
Suggestion: {
...at matches the model,  %\emph{SteinGAN} %\red{ %ccording to which shared inferences are cach...
                                                ^^                                             

46.) Line 96, column 148, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...ere a neural sampler is adaptively trained to  %approximate the likelihood gradient. Amortiz...
                                                ^^                                             

47.) Line 98, column 18, Rule ID: EN_QUOTES[3]
Message: Use a smart opening quote here: '“'.
Suggestion: “
...th the model distribution.  %In this way, we ``amortize SVGD'' using a neural network, which...
                                                ^^                                             
More info: https://en.wikipedia.org/wiki/Smart_quote#Electronic_documents

48.) Line 98, column 139, Rule ID: WHITESPACE_RULE
Message: Possible typo: you repeated a whitespace
Suggestion:  
...thod to adaptively improve its own efficiency   %Our method, which we call \emph{SteinGAN}, m...
                                                ^^^                                             

49.) Line 109, column 100, Rule ID: AFFORD_VB[1]
Message: This verb is used with the infinitive: 'to step'
Suggestion: to step
...s in CD.  However, it is difficult to choose step size and converge slow???   
                                                ^^^^                             
Time: 3635ms for 61 sentences (16.8 sentences/sec)

